Query-Focused Extractive Video Summarization

Video data is explosively growing. As a result of the "big video data", intelligent algorithms for automatic video summarization have re-emerged as a pressing need. We develop a probabilistic model, Sequential and Hierarchical Determinantal Point Process (SH-DPP), for query-focused extractive video summarization. Given a user query and a long video sequence, our algorithm returns a summary by selecting key shots from the video. The decision to include a shot in the summary depends on the shot's relevance to the user query and importance in the context of the video, jointly. We verify our approach on two densely annotated video datasets. The query-focused video summarization is particularly useful for search engines, e.g., to display snippets of videos.

==> Background.tex <==
% !TEX root = main.tex
\section{Background Review}
In this section of the paper, we overview the required background and notation followed by details of the approach. Our model extends sequential-DPP [] by adding another layer and making a second-order sequential-DPP. Therefore, we concisely review it and then proceed to details of our system.
\subsection{DPP}
\label{subsec:DPP}
[The coincidence approach to stochastic point processes] first introduced DPP, characterizing Pauli's exclusion principle, i.e. no two identical particles can occupy same quantum state at the same time. This makes DPP suitable for enforcing diversity which is an appealing property in variety of applications such as document summarization [], image search and ranking [], etc.\\
Let $\cal Y$ $= \{1,2,\dots,N\}$ be a ground set of items. In the simplest case, a DPP defines a discrete probability distribution. for $y \in \cal Y$ we have:\\
\begin{equation}
P(Y=y) = \frac{\det(\mat{L}_y)}{\det(\mat{L}+\mat{I})}
\end{equation} 
Where $\mat{I}$ is identity matrix, $\mat{L} \in \mathbb{S}^{N \times N}$ is the semidefinite kernel matrix induced by DPP parameters, and $\mat{L}_y$ is sub-matrix with rows and columns corresponding to the indices of subset $y$. Determinant function models pairwise repulsion, hence the most diverse subset of $\cal Y$, $y^*$, is the subset with maximum probability:\\
\begin{equation}
y^* = \argmax_y P(Y=y) = \argmax_y \det(\mat{L}_y)
\label{equ:vanillaDPP}
\end{equation}
